Classical Pre-Training of Large Shallow Parametrized Quantum Circuits through Pauli Propagation and deployment on Quantum Hardware

Scaling parametrized quantum circuits to a larger number of qubits is a central challenge in Quantum Machine Learning: gradient estimation via the parameter-shift rule quickly becomes prohibitively expensive, while gradient-free optimizers offer limited convergence guarantees. We apply the Pauli propagation framework to a broad class of Quantum Machine Learning problems in which the loss is expressed as a function of expectation values of the circuit's observables, while keeping the relevant quantity of interest, such as the quantum state or its samples, classically intractable to compute. By propagating the observables backward through the circuit, we obtain an explicit parametric expression for the loss that can be minimized entirely on classical hardware. We also present complementary strategies to make propagation tractable at large scale, including weight-based and degree-based truncations and pruning heuristics. We demonstrate the approach on two benchmarks run on 64-qubit circuits: Variational Quantum Eigensolver on a two-dimensional Ising model, and training of a discrete-type generative model for binary images. In both cases, the classically pre-trained parameters are deployed on the IBM quantum processor ibm_berlin. For generative learning, we additionally show that the circuits considered here require substantially fewer parametrized gates than IQP-style ans\"atze, reducing transpilation overhead and making deployment on current quantum hardware feasible.

==> tikz/qc.tex <==
% VQE quantum circuit: N qubits prepared in |0>^N, evolved by parameterised
% unitary U(theta), then measured.  Vertical slices label the state before and
% after U.  wire types={n,...} suppresses the input wire on the left.
\begin{quantikz}[row sep={0.5cm,between origins}, wire types={n,n,n,n}]
	 & [-.1cm] \lstick{$|0\rangle$}\slice[style={draw=gray}, label style={pos=1, anchor=north}]{$|0\rangle^{\otimes N}$} &
	\gate[4, style={fill=secondarycolor!30}]{\,\, U(\vec{\theta}) \,\,}\qw
	\slice[style={draw=gray}, label style={pos=1, anchor=north}]{\hspace*{0.5cm}$U(\vec{\theta})|0\rangle^{\otimes N}$}
	 & \qw                                                                                                               & [-.5cm] \meter{}                                 \\
	 & \lstick{$|0\rangle$}                                                                                              & \qw              & \qw & \meter{}                \\
	 & \lstick{\raisebox{.2cm}{\vdots}}\quad                                                                             &                  &     & \raisebox{.2cm}{\vdots} \\
	 & \lstick{$|0\rangle$}                                                                                              & \qw              & \qw & \meter{}
\end{quantikz}

